Stein Variational Probabilistic Roadmaps

Efficient and reliable generation of global path plans are necessary for safe execution and deployment of autonomous systems. In order to generate planning graphs which adequately resolve the topology of a given environment, many sampling-based motion planners resort to coarse, heuristically-driven strategies which often fail to generalize to new and varied surroundings. Further, many of these approaches are not designed to contend with partial-observability. We posit that such uncertainty in environment geometry can, in fact, help drive the sampling process in generating feasible, and probabilistically-safe planning graphs. We propose a method for Probabilistic Roadmaps which relies on particle-based Variational Inference to efficiently cover the posterior distribution over feasible regions in configuration space. Our approach, Stein Variational Probabilistic Roadmap (SV-PRM), results in sample-efficient generation of planning-graphs and large improvements over traditional sampling approaches. We demonstrate the approach on a variety of challenging planning problems, including real-world probabilistic occupancy maps and high-dof manipulation problems common in robotics.

==> figs/bhm_filmstrip.tex <==
% !TEX root = ../root.tex

\setlength{\fboxrule}{0pt}
\setlength{\fboxsep}{0pt}

\begin{figure*}[!ht]
\newlength{\envwidth}
\setlength{\envwidth}{0.19\linewidth}
\centering
\hfill
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/bhm_filmstrip/00.pdf}}
\end{subfigure}
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/bhm_filmstrip/05.pdf}}
\end{subfigure}
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/bhm_filmstrip/10.pdf}}
\end{subfigure}
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/bhm_filmstrip/55.pdf}}
\end{subfigure}
\begin{subfigure}{\envwidth}
\fbox{\includegraphics[height=\linewidth]{figs/bhm_filmstrip/101.pdf}}
\end{subfigure}
\hfill

\caption{
Stein Variational PRMs use a particle-based variational inference algorithm to match the probabilistic occupancy map distribution.
}
\label{fig:bhm_filmstrip}
\vspace{-1\baselineskip}
\end{figure*}

% restore defaults
\setlength{\fboxrule}{0.2pt}
\setlength{\fboxsep}{3pt}

==> figs/toy2d_panels_old.tex <==
\setlength{\fboxrule}{0pt}
\setlength{\fboxsep}{0pt}

\begin{figure}[!t]
\newlength{\heatmapwidth}
\setlength{\heatmapwidth}{0.31\linewidth}
\centering

\fbox{\includegraphics[width=\heatmapwidth]{figs/toy2d/num_particles=100,uniform+rej.pdf}}
\hfill
\fbox{\includegraphics[width=\heatmapwidth]{figs/toy2d/num_particles=100,halton+rej.pdf}}
\hfill
\fbox{\includegraphics[width=\heatmapwidth]{figs/toy2d/num_particles=100,uniform+rej+svgd.pdf}}

\medskip

\fbox{\includegraphics[width=\heatmapwidth]{figs/toy2d/num_particles=250,uniform+rej.pdf}}
\hfill
\fbox{\includegraphics[width=\heatmapwidth]{figs/toy2d/num_particles=250,halton+rej.pdf}}
\hfill
\fbox{\includegraphics[width=\heatmapwidth]{figs/toy2d/num_particles=250,uniform+rej+svgd.pdf}}

\caption{
\checkerboard roadmaps generated with different sampling strategies and number of samples.
The planning query consists of the start (green) and goal (red),
and the shortest path (blue) is visualized if it exists.
(Left) Uniform sampling with rejection.
(Center) Halton sampling with rejection.
(Right) Stein Variational PRM, initialized with the left column of particles.
(Top) 100 particles.
(Bottom) 250 particles.
Best viewed digitally.
%Top: low particle regime (num_particles=100) uniform+rejection sampling, halton+rejection sampling, uniform+rejection+svgd.
%Bottom: high particle regime (num_particles=250) uniform+rejection sampling, halton+rejection sampling, uniform+rejection+svgd
% \slnote{Mention that SV-PRM is initialized using the corresponding sample distribution in the first column.}
}
\label{fig:toy2dqual}
% \vspace{-1\baselineskip}
\end{figure}

% restore defaults
\setlength{\fboxrule}{0.2pt}
\setlength{\fboxsep}{3pt}

==> inputs/z_graveyard.tex <==
\input{tables/toy2d_pathlength}
\input{tables/toy2d_collisionchecks}


==> tables/toy2d_collisionchecks.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}lcccccccc@{}}\toprule
&  PRM(U) & PRM(H) & PRM(U+Rej) & PRM(H+Rej) & SV-PRM(U) & SV-PRM(H) & SV-PRM(U+Rej) & SV-PRM(H+Rej) \\ \midrule
Low        & $1173 \pm 150$ & $ n/a $        & $3454 \pm 173 $ & $4088 \pm 00$ & $3963 \pm 110 $ & $4770 \pm 00$ & $3846 \pm 88$ & $3769 \pm 00$ \\
High       & $6516 \pm 304$ & $ 6465 \pm 00$ & $22336 \pm 645 $ & $18435 \pm 00$ & $ 21758 \pm 270 $ & $22969 \pm 00$ & $22025 \pm 441$ & $21384 \pm 00$ \\
\bottomrule
\end{tabular}
\caption{
Collision Checks
}
\label{tab:toy2d_collision}
\end{table*}

==> tables/toy2d_pathlength.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}lcccccccc@{}}\toprule
&  PRM(U) & PRM(H) & PRM(U+Rej) & PRM(H+Rej) & SV-PRM(U) & SV-PRM(H) & SV-PRM(U+Rej) & SV-PRM(H+Rej) \\ \midrule
Low        & $34.62 \pm .05$ & $ n/a $          & $34.93 \pm .41$ & $34.63 \pm .00$ & $35.12 \pm .16$ & $35.46 \pm  .00$ & $35.43 \pm  .00$ & $35.43 \pm .00$ \\
High       & $34.33 \pm .03$ & $ 34.06 \pm 0.0$ & $33.25 \pm .07$ & $32.59 \pm .00$ & $33.09 \pm .06$ & $32.92 \pm .03$ & $33.03 \pm .00$ & $33.03 \pm .00$ \\
\bottomrule
\end{tabular}
\caption{
Path Length
}
\label{tab:toy2d_pathlength}
\end{table*}
